Masked Thought: Simply Masking Partial Reasoning Steps Can Improve Mathematical Reasoning Learning of Language Models

In reasoning tasks, even a minor error can cascade into inaccurate results, leading to suboptimal performance of large language models in such domains. Earlier fine-tuning approaches sought to mitigate this by leveraging more precise supervisory signals from human labeling, larger models, or self-sampling, although at a high cost. Conversely, we develop a method that avoids external resources, relying instead on introducing perturbations to the input. Our training approach randomly masks certain tokens within the chain of thought, a technique we found to be particularly effective for reasoning tasks. When applied to fine-tuning with GSM8K on Llama-2-7B, this method achieved a 5\% improvement in GSM8K accuracy and a 10\% improvement in GSM-IC accuracy over standard supervised fine-tuning with a few codes modified. Furthermore, it is complementary to existing methods. When integrated with related explicit data augmentation methods, it leads to improvements across five datasets of various augmentation methods, as well as two different base models. We further investigate the mechanisms behind this improvement through case studies and quantitative analysis, suggesting that our approach may provide superior support for the model in capturing long-distance dependencies, especially those related to questions. This enhancement could deepen understanding of the premises in questions and prior steps. Our code is available at Github.

==> nothing <==
\begin{thebibliography}{66}
\expandafter\ifx\csname natexlab\endcsname\relax\def\natexlab#1{#1}\fi

\bibitem[{Achiam et~al.(2023)Achiam, Adler, Agarwal, Ahmad, Akkaya, Aleman, Almeida, Altenschmidt, Altman, Anadkat et~al.}]{gpt4}
Josh Achiam, Steven Adler, Sandhini Agarwal, Lama Ahmad, Ilge Akkaya, Florencia~Leoni Aleman, Diogo Almeida, Janko Altenschmidt, Sam Altman, Shyamal Anadkat, et~al. 2023.
\newblock Gpt-4 technical report.
\newblock \emph{arXiv preprint arXiv:2303.08774}.

\bibitem[{An et~al.(2023)An, Ma, Lin, Zheng, Lou, and Chen}]{An2023LearningFM}
Shengnan An, Zexiong Ma, Zeqi Lin, Nanning Zheng, Jian-Guang Lou, and Weizhu Chen. 2023.
\newblock \href {https://api.semanticscholar.org/CorpusID:264813981} {Learning from mistakes makes llm better reasoner}.
\newblock \emph{ArXiv}, abs/2310.20689.

\bibitem[{Azerbayev et~al.(2023)Azerbayev, Schoelkopf, Paster, Santos, McAleer, Jiang, Deng, Biderman, and Welleck}]{llemma}
Zhangir Azerbayev, Hailey Schoelkopf, Keiran Paster, Marco~Dos Santos, Stephen McAleer, Albert~Q Jiang, Jia Deng, Stella Biderman, and Sean Welleck. 2023.
\newblock Llemma: An open language model for mathematics.
\newblock \emph{arXiv preprint arXiv:2310.10631}.

\bibitem[{Bao et~al.(2020)Bao, Dong, Wei, Wang, Yang, Liu, Wang, Piao, Gao, Zhou, and Hon}]{Bao2020UniLMv2PL}
Hangbo Bao, Li~Dong, Furu Wei, Wenhui Wang, Nan Yang, Xiaodong Liu, Yu~Wang, Songhao Piao, Jianfeng Gao, Ming Zhou, and Hsiao-Wuen Hon. 2020.
\newblock \href {https://api.semanticscholar.org/CorpusID:211572655} {Unilmv2: Pseudo-masked language models for unified language model pre-training}.
\newblock In \emph{International Conference on Machine Learning}.

\bibitem[{Bengio et~al.(2015)Bengio, Vinyals, Jaitly, and Shazeer}]{bengio2015scheduled}
Samy Bengio, Oriol Vinyals, Navdeep Jaitly, and Noam Shazeer. 2015.
\newblock Scheduled sampling for sequence prediction with recurrent neural networks.
\newblock \emph{Advances in neural information processing systems}, 28.

\bibitem[{Besta et~al.(2023)Besta, Blach, Kubicek, Gerstenberger, Gianinazzi, Gajda, Lehmann, Podstawski, Niewiadomski, Nyczyk et~al.}]{besta2023graph}
Maciej Besta, Nils Blach, Ales Kubicek, Robert Gerstenberger, Lukas Gianinazzi, Joanna Gajda, Tomasz Lehmann, Michal Podstawski, Hubert Niewiadomski, Piotr Nyczyk, et~al. 2023.
\newblock Graph of thoughts: Solving elaborate problems with large language models.
\newblock \emph{arXiv preprint arXiv:2308.09687}.

\bibitem[{Chen et~al.(2023{\natexlab{a}})Chen, Wang, Jin, Dong, Dong, Cao, Liu, and Yan}]{chen2023semi}
Changyu Chen, Xiting Wang, Yiqiao Jin, Victor~Ye Dong, Li~Dong, Jie Cao, Yi~Liu, and Rui Yan. 2023{\natexlab{a}}.
\newblock Semi-offline reinforcement learning for optimized text generation.
\newblock \emph{arXiv preprint arXiv:2306.09712}.

\bibitem[{Chen et~al.(2023{\natexlab{b}})Chen, Tam, Raffel, Bansal, and Yang}]{chen2023empirical}
Jiaao Chen, Derek Tam, Colin Raffel, Mohit Bansal, and Diyi Yang. 2023{\natexlab{b}}.
\newblock An empirical survey of data augmentation for limited data learning in nlp.
\newblock \emph{Transactions of the Association for Computational Linguistics}, 11:191--211.

\bibitem[{Chen et~al.(2022)Chen, Ma, Wang, and Cohen}]{chen2022program}
Wenhu Chen, Xueguang Ma, Xinyi Wang, and William~W Cohen. 2022.
\newblock Program of thoughts prompting: Disentangling computation from reasoning for numerical reasoning tasks.
\newblock \emph{arXiv preprint arXiv:2211.12588}.

\bibitem[{Chen et~al.(2024)Chen, Chi, Wang, and Zhou}]{chen2024premise}
Xinyun Chen, Ryan~A Chi, Xuezhi Wang, and Denny Zhou. 2024.
\newblock Premise order matters in reasoning with large language models.
\newblock \emph{arXiv preprint arXiv:2402.08939}.

\bibitem[{Cheng et~al.(2018)Cheng, Tu, Meng, Zhai, and Liu}]{Cheng2018TowardsRN}
Yong Cheng, Zhaopeng Tu, Fandong Meng, Junjie Zhai, and Yang Liu. 2018.
\newblock \href {https://api.semanticscholar.org/CorpusID:21715690} {Towards robust neural machine translation}.
\newblock \emph{ArXiv}, abs/1805.06130.

\bibitem[{Cobbe et~al.(2021)Cobbe, Kosaraju, Bavarian, Chen, Jun, Kaiser, Plappert, Tworek, Hilton, Nakano et~al.}]{cobbe2021training}
Karl Cobbe, Vineet Kosaraju, Mohammad Bavarian, Mark Chen, Heewoo Jun, Lukasz Kaiser, Matthias Plappert, Jerry Tworek, Jacob Hilton, Reiichiro Nakano, et~al. 2021.
\newblock Training verifiers to solve math word problems.
\newblock \emph{arXiv preprint arXiv:2110.14168}.

\bibitem[{Devlin et~al.(2019)Devlin, Chang, Lee, and Toutanova}]{Devlin2019BERTPO}
Jacob Devlin, Ming-Wei Chang, Kenton Lee, and Kristina Toutanova. 2019.
\newblock \href {https://api.semanticscholar.org/CorpusID:52967399} {Bert: Pre-training of deep bidirectional transformers for language understanding}.
\newblock In \emph{North American Chapter of the Association for Computational Linguistics}.

\bibitem[{Dziri et~al.(2023)Dziri, Lu, Sclar, Li, Jian, Lin, West, Bhagavatula, Bras, Hwang, Sanyal, Welleck, Ren, Ettinger, Harchaoui, and Choi}]{Dziri2023FaithAF}
Nouha Dziri, Ximing Lu, Melanie Sclar, Xiang~Lorraine Li, Liwei Jian, Bill~Yuchen Lin, Peter West, Chandra Bhagavatula, Ronan~Le Bras, Jena~D. Hwang, Soumya Sanyal, Sean Welleck, Xiang Ren, Allyson Ettinger, Za{\"i}d Harchaoui, and Yejin Choi. 2023.
\newblock \href {https://api.semanticscholar.org/CorpusID:258967391} {Faith and fate: Limits of transformers on compositionality}.
\newblock \emph{ArXiv}, abs/2305.18654.

\bibitem[{Fadaee et~al.(2017)Fadaee, Bisazza, and Monz}]{fadaee2017data}
Marzieh Fadaee, Arianna Bisazza, and Christof Monz. 2017.
\newblock Data augmentation for low-resource neural machine translation.
\newblock \emph{arXiv preprint arXiv:1705.00440}.

\bibitem[{Fu et~al.(2022)Fu, Peng, Sabharwal, Clark, and Khot}]{fu2022complexity}
Yao Fu, Hao Peng, Ashish Sabharwal, Peter Clark, and Tushar Khot. 2022.
\newblock Complexity-based prompting for multi-step reasoning.
\newblock \emph{arXiv preprint arXiv:2210.00720}.

\bibitem[{Gal and Ghahramani(2015)}]{Gal2015ATG}
Yarin Gal and Zoubin Ghahramani. 2015.
\newblock \href {https://api.semanticscholar.org/CorpusID:15953218} {A theoretically grounded application of dropout in recurrent neural networks}.
\newblock In \emph{Neural Information Processing Systems}.

\bibitem[{Gou et~al.(2023)Gou, Shao, Gong, Shen, Yang, Huang, Duan, and Chen}]{Gou2023ToRAAT}
Zhibin Gou, Zhihong Shao, Yeyun Gong, Yelong Shen, Yujiu Yang, Minlie Huang, Nan Duan, and Weizhu Chen. 2023.
\newblock \href {https://api.semanticscholar.org/CorpusID:263310365} {Tora: A tool-integrated reasoning agent for mathematical problem solving}.
\newblock \emph{ArXiv}, abs/2309.17452.

\bibitem[{Guo et~al.(2020{\natexlab{a}})Guo, Kim, and Rush}]{guo2020sequence}
Demi Guo, Yoon Kim, and Alexander~M Rush. 2020{\natexlab{a}}.
\newblock Sequence-level mixed sample data augmentation.
\newblock \emph{arXiv preprint arXiv:2011.09039}.

\bibitem[{Guo et~al.(2020{\natexlab{b}})Guo, Kim, and Rush}]{Guo2020SequencelevelMS}
Demi Guo, Yoon Kim, and Alexander~M. Rush. 2020{\natexlab{b}}.
\newblock \href {https://api.semanticscholar.org/CorpusID:226262205} {Sequence-level mixed sample data augmentation}.
\newblock In \emph{Conference on Empirical Methods in Natural Language Processing}.

\bibitem[{Hendrycks et~al.(2021)Hendrycks, Burns, Kadavath, Arora, Basart, Tang, Song, and Steinhardt}]{hendrycks2021measuring}
Dan Hendrycks, Collin Burns, Saurav Kadavath, Akul Arora, Steven Basart, Eric Tang, Dawn Song, and Jacob Steinhardt. 2021.
\newblock Measuring mathematical problem solving with the math dataset.
\newblock \emph{arXiv preprint arXiv:2103.03874}.

\bibitem[{Huang et~al.(2023{\natexlab{a}})Huang, Chen, Mishra, Zheng, Yu, Song, and Zhou}]{huang2023large}
Jie Huang, Xinyun Chen, Swaroop Mishra, Huaixiu~Steven Zheng, Adams~Wei Yu, Xinying Song, and Denny Zhou. 2023{\natexlab{a}}.
\newblock Large language models cannot self-correct reasoning yet.
\newblock \emph{arXiv preprint arXiv:2310.01798}.

\bibitem[{Huang et~al.(2023{\natexlab{b}})Huang, Yu, Ma, Zhong, Feng, Wang, Chen, Peng, Feng, Qin, and Liu}]{huang2023survey}
Lei Huang, Weijiang Yu, Weitao Ma, Weihong Zhong, Zhangyin Feng, Haotian Wang, Qianglong Chen, Weihua Peng, Xiaocheng Feng, Bing Qin, and Ting Liu. 2023{\natexlab{b}}.
\newblock \href {http://arxiv.org/abs/2311.05232} {A survey on hallucination in large language models: Principles, taxonomy, challenges, and open questions}.

\bibitem[{Jain et~al.(2023)Jain, yeh Chiang, Wen, Kirchenbauer, Chu, Somepalli, Bartoldson, Kailkhura, Schwarzschild, Saha, Goldblum, Geiping, and Goldstein}]{jain2023neftune}
Neel Jain, Ping yeh Chiang, Yuxin Wen, John Kirchenbauer, Hong-Min Chu, Gowthami Somepalli, Brian~R. Bartoldson, Bhavya Kailkhura, Avi Schwarzschild, Aniruddha Saha, Micah Goldblum, Jonas Geiping, and Tom Goldstein. 2023.
\newblock \href {http://arxiv.org/abs/2310.05914} {Neftune: Noisy embeddings improve instruction finetuning}.

\bibitem[{Jiang et~al.(2023)Jiang, Sablayrolles, Mensch, Bamford, Chaplot, Casas, Bressand, Lengyel, Lample, Saulnier et~al.}]{mistral}
Albert~Q Jiang, Alexandre Sablayrolles, Arthur Mensch, Chris Bamford, Devendra~Singh Chaplot, Diego de~las Casas, Florian Bressand, Gianna Lengyel, Guillaume Lample, Lucile Saulnier, et~al. 2023.
\newblock Mistral 7b.
\newblock \emph{arXiv preprint arXiv:2310.06825}.

\bibitem[{Kedzie and McKeown(2019)}]{Kedzie2019AGS}
Chris Kedzie and Kathleen McKeown. 2019.
\newblock \href {https://api.semanticscholar.org/CorpusID:207847447} {A good sample is hard to find: Noise injection sampling and self-training for neural language generation models}.
\newblock In \emph{International Conference on Natural Language Generation}.

\bibitem[{Khona et~al.(2024)Khona, Okawa, Hula, Ramesh, Nishi, Dick, Lubana, and Tanaka}]{Khona2024TowardsAU}
Mikail Khona, Maya Okawa, Jan Hula, Rahul Ramesh, Kento Nishi, Robert Dick, Ekdeep~Singh Lubana, and Hidenori Tanaka. 2024.
\newblock Towards an understanding of stepwise inference in transformers: A synthetic graph navigation model.
\newblock \emph{arXiv preprint arXiv:2402.07757}.

\bibitem[{Kojima et~al.(2022)Kojima, Gu, Reid, Matsuo, and Iwasawa}]{kojima2022large}
Takeshi Kojima, Shixiang~Shane Gu, Machel Reid, Yutaka Matsuo, and Yusuke Iwasawa. 2022.
\newblock Large language models are zero-shot reasoners.
\newblock \emph{Advances in neural information processing systems}, 35:22199--22213.

\bibitem[{Lample et~al.(2017)Lample, Conneau, Denoyer, and Ranzato}]{lample2017unsupervised}
Guillaume Lample, Alexis Conneau, Ludovic Denoyer, and Marc'Aurelio Ranzato. 2017.
\newblock Unsupervised machine translation using monolingual corpora only.
\newblock \emph{arXiv preprint arXiv:1711.00043}.

\bibitem[{Li et~al.(2023{\natexlab{a}})Li, Hammoud, Itani, Khizbullin, and Ghanem}]{li2023camel}
Guohao Li, Hasan Abed Al~Kader Hammoud, Hani Itani, Dmitrii Khizbullin, and Bernard Ghanem. 2023{\natexlab{a}}.
\newblock Camel: Communicative agents for" mind" exploration of large scale language model society.
\newblock \emph{arXiv preprint arXiv:2303.17760}.

\bibitem[{Li et~al.(2023{\natexlab{b}})Li, Zhang, Dubois, Taori, Gulrajani, Guestrin, Liang, and Hashimoto}]{alpaca_eval}
Xuechen Li, Tianyi Zhang, Yann Dubois, Rohan Taori, Ishaan Gulrajani, Carlos Guestrin, Percy Liang, and Tatsunori~B. Hashimoto. 2023{\natexlab{b}}.
\newblock Alpacaeval: An automatic evaluator of instruction-following models.
\newblock \url{https://github.com/tatsu-lab/alpaca_eval}.

\bibitem[{Li et~al.(2022)Li, Lin, Zhang, Fu, Chen, Lou, and Chen}]{Li2022MakingLM}
Yifei Li, Zeqi Lin, Shizhuo Zhang, Qiang Fu, B.~Chen, Jian-Guang Lou, and Weizhu Chen. 2022.
\newblock \href {https://api.semanticscholar.org/CorpusID:259370847} {Making language models better reasoners with step-aware verifier}.
\newblock In \emph{Annual Meeting of the Association for Computational Linguistics}.

\bibitem[{Liao et~al.(2024)Liao, Luo, Li, Wu, and Fan}]{Liao2024MARIOMR}
Minpeng Liao, Wei Luo, Chengxi Li, Jing Wu, and Kai Fan. 2024.
\newblock \href {https://api.semanticscholar.org/CorpusID:267028217} {Mario: Math reasoning with code interpreter output - a reproducible pipeline}.
\newblock \emph{ArXiv}, abs/2401.08190.

\bibitem[{Lightman et~al.(2023)Lightman, Kosaraju, Burda, Edwards, Baker, Lee, Leike, Schulman, Sutskever, and Cobbe}]{Lightman2023LetsVS}
Hunter Lightman, Vineet Kosaraju, Yura Burda, Harrison Edwards, Bowen Baker, Teddy Lee, Jan Leike, John Schulman, Ilya Sutskever, and Karl Cobbe. 2023.
\newblock \href {https://api.semanticscholar.org/CorpusID:258987659} {Let's verify step by step}.
\newblock \emph{ArXiv}, abs/2305.20050.

\bibitem[{Ling et~al.(2017)Ling, Yogatama, Dyer, and Blunsom}]{ling2017program}
Wang Ling, Dani Yogatama, Chris Dyer, and Phil Blunsom. 2017.
\newblock Program induction by rationale generation: Learning to solve and explain algebraic word problems.
\newblock \emph{arXiv preprint arXiv:1705.04146}.

\bibitem[{Liu et~al.(2022)Liu, Ash, Goel, Krishnamurthy, and Zhang}]{Liu2022TransformersLS}
Bingbin Liu, Jordan~T. Ash, Surbhi Goel, Akshay Krishnamurthy, and Cyril Zhang. 2022.
\newblock \href {https://api.semanticscholar.org/CorpusID:252992725} {Transformers learn shortcuts to automata}.
\newblock \emph{ArXiv}, abs/2210.10749.

\bibitem[{Liu et~al.(2023)Liu, Bubeck, Eldan, Kulkarni, Li, Nguyen, Ward, and Zhang}]{liu2023tinygsm}
Bingbin Liu, Sebastien Bubeck, Ronen Eldan, Janardhan Kulkarni, Yuanzhi Li, Anh Nguyen, Rachel Ward, and Yi~Zhang. 2023.
\newblock Tinygsm: achieving> 80\% on gsm8k with small language models.
\newblock \emph{arXiv preprint arXiv:2312.09241}.

\bibitem[{Luo et~al.(2023)Luo, Sun, Xu, Zhao, Lou, Tao, Geng, Lin, Chen, and Zhang}]{luo2023wizardmath}
Haipeng Luo, Qingfeng Sun, Can Xu, Pu~Zhao, Jianguang Lou, Chongyang Tao, Xiubo Geng, Qingwei Lin, Shifeng Chen, and Dongmei Zhang. 2023.
\newblock Wizardmath: Empowering mathematical reasoning for large language models via reinforced evol-instruct.
\newblock \emph{arXiv preprint arXiv:2308.09583}.

\bibitem[{Mihaylova and Martins(2019)}]{mihaylova2019scheduled}
Tsvetomila Mihaylova and Andr{\'e}~FT Martins. 2019.
\newblock Scheduled sampling for transformers.
\newblock \emph{arXiv preprint arXiv:1906.07651}.

\bibitem[{Prystawski et~al.(2023)Prystawski, Li, and Goodman}]{Prystawski2023WhyTS}
Ben Prystawski, Michael~Y. Li, and Noah~D. Goodman. 2023.
\newblock \href {https://api.semanticscholar.org/CorpusID:258048648} {Why think step-by-step? reasoning emerges from the locality of experience}.
\newblock \emph{ArXiv}, abs/2304.03843.

\bibitem[{Schulman et~al.(2017)Schulman, Wolski, Dhariwal, Radford, and Klimov}]{schulman2017proximal}
John Schulman, Filip Wolski, Prafulla Dhariwal, Alec Radford, and Oleg Klimov. 2017.
\newblock Proximal policy optimization algorithms.
\newblock \emph{arXiv preprint arXiv:1707.06347}.

\bibitem[{Schwab and Karlen(2019)}]{schwab2019cxplain}
Patrick Schwab and Walter Karlen. 2019.
\newblock {CXPlain: Causal Explanations for Model Interpretation under Uncertainty}.
\newblock In \emph{{Advances in Neural Information Processing Systems (NeurIPS)}}.

\bibitem[{Shi et~al.(2023)Shi, Chen, Misra, Scales, Dohan, Chi, Sch{\"a}rli, and Zhou}]{shi2023large}
Freda Shi, Xinyun Chen, Kanishka Misra, Nathan Scales, David Dohan, Ed~H Chi, Nathanael Sch{\"a}rli, and Denny Zhou. 2023.
\newblock Large language models can be easily distracted by irrelevant context.
\newblock In \emph{International Conference on Machine Learning}, pages 31210--31227. PMLR.

\bibitem[{Singh et~al.(2023)Singh, Co-Reyes, Agarwal, Anand, Patil, Liu, Harrison, Lee, Xu, Parisi et~al.}]{singh2023beyond}
Avi Singh, John~D Co-Reyes, Rishabh Agarwal, Ankesh Anand, Piyush Patil, Peter~J Liu, James Harrison, Jaehoon Lee, Kelvin Xu, Aaron Parisi, et~al. 2023.
\newblock Beyond human data: Scaling self-training for problem-solving with language models.
\newblock \emph{arXiv preprint arXiv:2312.06585}.

\bibitem[{Sinha et~al.(2022)Sinha, Mandlekar, and Garg}]{stateDA}
Samarth Sinha, Ajay Mandlekar, and Animesh Garg. 2022.
\newblock S4rl: Surprisingly simple self-supervision for offline reinforcement learning in robotics.
\newblock In \emph{Conference on Robot Learning}, pages 907--917. PMLR.

\bibitem[{Srivastava et~al.(2014)Srivastava, Hinton, Krizhevsky, Sutskever, and Salakhutdinov}]{Srivastava2014DropoutAS}
Nitish Srivastava, Geoffrey~E. Hinton, Alex Krizhevsky, Ilya Sutskever, and Ruslan Salakhutdinov. 2014.
\newblock \href {https://api.semanticscholar.org/CorpusID:6844431} {Dropout: a simple way to prevent neural networks from overfitting}.
\newblock \emph{J. Mach. Learn. Res.}, 15:1929--1958.

\bibitem[{Su et~al.(2022)Su, Lee, Hsu, and Su}]{su-etal-2022-roberta}
Ming-Hsiang Su, Chin-Wei Lee, Chi-Lun Hsu, and Ruei-Cyuan Su. 2022.
\newblock \href {https://aclanthology.org/2022.rocling-1.8} {{R}o{BERT}a-based traditional {C}hinese medicine named entity recognition model}.
\newblock In \emph{Proceedings of the 34th Conference on Computational Linguistics and Speech Processing (ROCLING 2022)}, pages 61--66, Taipei, Taiwan. The Association for Computational Linguistics and Chinese Language Processing (ACLCLP).

\bibitem[{Taori et~al.(2023)Taori, Gulrajani, Zhang, Dubois, Li, Guestrin, Liang, and Hashimoto}]{taori2023stanford}
Rohan Taori, Ishaan Gulrajani, Tianyi Zhang, Yann Dubois, Xuechen Li, Carlos Guestrin, Percy Liang, and Tatsunori~B Hashimoto. 2023.
\newblock Stanford alpaca: An instruction-following llama model.

\bibitem[{Touvron et~al.(2023)Touvron, Martin, Stone, Albert, Almahairi, Babaei, Bashlykov, Batra, Bhargava, Bhosale et~al.}]{llama}
Hugo Touvron, Louis Martin, Kevin Stone, Peter Albert, Amjad Almahairi, Yasmine Babaei, Nikolay Bashlykov, Soumya Batra, Prajjwal Bhargava, Shruti Bhosale, et~al. 2023.
\newblock Llama 2: Open foundation and fine-tuned chat models.
\newblock \emph{arXiv preprint arXiv:2307.09288}.

\bibitem[{Uesato et~al.(2022)Uesato, Kushman, Kumar, Song, Siegel, Wang, Creswell, Irving, and Higgins}]{uesato2022solving}
Jonathan Uesato, Nate Kushman, Ramana Kumar, Francis Song, Noah Siegel, Lisa Wang, Antonia Creswell, Geoffrey Irving, and Irina Higgins. 2022.
\newblock Solving math word problems with process-and outcome-based feedback.
\newblock \emph{arXiv preprint arXiv:2211.14275}.

\bibitem[{Wang et~al.(2023{\natexlab{a}})Wang, Xu, Lan, Hu, Lan, Lee, and Lim}]{wang2023planandsolve}
Lei Wang, Wanyu Xu, Yihuai Lan, Zhiqiang Hu, Yunshi Lan, Roy Ka-Wei Lee, and Ee-Peng Lim. 2023{\natexlab{a}}.
\newblock Plan-and-solve prompting: Improving zero-shot chain-of-thought reasoning by large language models.
\newblock \emph{arXiv preprint arXiv:2305.04091}.

\bibitem[{Wang et~al.(2023{\natexlab{b}})Wang, Li, Shao, Xu, Dai, Li, Chen, Wu, and Sui}]{wang2023math}
Peiyi Wang, Lei Li, Zhihong Shao, RX~Xu, Damai Dai, Yifei Li, Deli Chen, Y~Wu, and Zhifang Sui. 2023{\natexlab{b}}.
\newblock Math-shepherd: A label-free step-by-step verifier for llms in mathematical reasoning.
\newblock \emph{arXiv preprint arXiv:2312.08935}.

\bibitem[{Wang et~al.(2018)Wang, Pham, Dai, and Neubig}]{Wang2018SwitchOutAE}
Xinyi Wang, Hieu Pham, Zihang Dai, and Graham Neubig. 2018.
\newblock \href {https://api.semanticscholar.org/CorpusID:52078335} {Switchout: an efficient data augmentation algorithm for neural machine translation}.
\newblock In \emph{Conference on Empirical Methods in Natural Language Processing}.

\bibitem[{Wang et~al.(2022)Wang, Wei, Schuurmans, Le, Chi, Narang, Chowdhery, and Zhou}]{wang2022self}
Xuezhi Wang, Jason Wei, Dale Schuurmans, Quoc Le, Ed~Chi, Sharan Narang, Aakanksha Chowdhery, and Denny Zhou. 2022.
\newblock Self-consistency improves chain of thought reasoning in language models.
\newblock \emph{arXiv preprint arXiv:2203.11171}.

\bibitem[{Wei et~al.(2022)Wei, Wang, Schuurmans, Bosma, Xia, Chi, Le, Zhou et~al.}]{Wei2022ChainOT}
Jason Wei, Xuezhi Wang, Dale Schuurmans, Maarten Bosma, Fei Xia, Ed~Chi, Quoc~V Le, Denny Zhou, et~al. 2022.
\newblock Chain-of-thought prompting elicits reasoning in large language models.
\newblock \emph{Advances in Neural Information Processing Systems}, 35:24824--24837.

\bibitem[{Wei and Zou(2019)}]{Wei2019EDAED}
Jason Wei and Kai Zou. 2019.
\newblock \href {https://api.semanticscholar.org/CorpusID:59523656} {Eda: Easy data augmentation techniques for boosting performance on text classification tasks}.
\newblock In \emph{Conference on Empirical Methods in Natural Language Processing}.

\bibitem[{Xi et~al.(2024)Xi, Chen, Hong, Jin, Zheng, He, Ding, Liu, Guo, Wang et~al.}]{Xi2024TrainingLL}
Zhiheng Xi, Wenxiang Chen, Boyang Hong, Senjie Jin, Rui Zheng, Wei He, Yiwen Ding, Shichun Liu, Xin Guo, Junzhe Wang, et~al. 2024.
\newblock Training large language models for reasoning through reverse curriculum reinforcement learning.
\newblock \emph{arXiv preprint arXiv:2402.05808}.

\bibitem[{Xie et~al.(2022)Xie, Lv, Xia, Wu, Qin, Liu, and Yan}]{xie2022targetside}
Shufang Xie, Ang Lv, Yingce Xia, Lijun Wu, Tao Qin, Tie-Yan Liu, and Rui Yan. 2022.
\newblock \href {https://openreview.net/forum?id=pz1euXohm4H} {Target-side input augmentation for sequence to sequence generation}.
\newblock In \emph{International Conference on Learning Representations}.

\bibitem[{Xie et~al.(2016)Xie, Wang, Li, L{\'e}vy, Nie, Jurafsky, and Ng}]{smoothing}
Ziang Xie, Sida~I Wang, Jiwei Li, Daniel L{\'e}vy, Aiming Nie, Dan Jurafsky, and Andrew~Y Ng. 2016.
\newblock Data noising as smoothing in neural network language models.
\newblock In \emph{International Conference on Learning Representations}.

\bibitem[{Yao et~al.(2023)Yao, Yu, Zhao, Shafran, Griffiths, Cao, and Narasimhan}]{yao2023tree}
Shunyu Yao, Dian Yu, Jeffrey Zhao, Izhak Shafran, Thomas~L Griffiths, Yuan Cao, and Karthik Narasimhan. 2023.
\newblock Tree of thoughts: Deliberate problem solving with large language models.
\newblock \emph{arXiv preprint arXiv:2305.10601}.

\bibitem[{Yao et~al.(2022)Yao, Zhao, Yu, Du, Shafran, Narasimhan, and Cao}]{yao2022react}
Shunyu Yao, Jeffrey Zhao, Dian Yu, Nan Du, Izhak Shafran, Karthik Narasimhan, and Yuan Cao. 2022.
\newblock React: Synergizing reasoning and acting in language models.
\newblock \emph{arXiv preprint arXiv:2210.03629}.

\bibitem[{Yu et~al.(2023)Yu, Jiang, Shi, Yu, Liu, Zhang, Kwok, Li, Weller, and Liu}]{yu2023metamath}
Longhui Yu, Weisen Jiang, Han Shi, Jincheng Yu, Zhengying Liu, Yu~Zhang, James~T Kwok, Zhenguo Li, Adrian Weller, and Weiyang Liu. 2023.
\newblock Metamath: Bootstrap your own mathematical questions for large language models.
\newblock \emph{arXiv preprint arXiv:2309.12284}.

\bibitem[{Yuan et~al.(2023)Yuan, Yuan, Li, Dong, Tan, and Zhou}]{yuan2023RFT}
Zheng Yuan, Hongyi Yuan, Chengpeng Li, Guanting Dong, Chuanqi Tan, and Chang Zhou. 2023.
\newblock Scaling relationship on learning mathematical reasoning with large language models.
\newblock \emph{arXiv preprint arXiv:2308.01825}.

\bibitem[{Yue et~al.(2023)Yue, Qu, Zhang, Fu, Huang, Sun, Su, and Chen}]{yue2023mammoth}
Xiang Yue, Xingwei Qu, Ge~Zhang, Yao Fu, Wenhao Huang, Huan Sun, Yu~Su, and Wenhu Chen. 2023.
\newblock Mammoth: Building math generalist models through hybrid instruction tuning.
\newblock \emph{arXiv preprint arXiv:2309.05653}.

\bibitem[{Zelikman et~al.(2022)Zelikman, Wu, Mu, and Goodman}]{zelikman2022star}
Eric Zelikman, Yuhuai Wu, Jesse Mu, and Noah Goodman. 2022.
\newblock Star: Bootstrapping reasoning with reasoning.
\newblock \emph{Advances in Neural Information Processing Systems}, 35:15476--15488.

\bibitem[{Zhang et~al.(2015)Zhang, Zhao, and LeCun}]{Zhang2015CharacterlevelCN}
Xiang Zhang, Junbo~Jake Zhao, and Yann LeCun. 2015.
\newblock \href {https://api.semanticscholar.org/CorpusID:368182} {Character-level convolutional networks for text classification}.
\newblock In \emph{Neural Information Processing Systems}.

\end{thebibliography}


==> src/discussion_limitation.tex <==
\section{Discusion}
\subsection{Relation to scheduled sampling}
~\label{sec:eb}
Implicitly mixing model prediction distribution with data distribution: With the powerful language modeling capabilities of current large-parameter models, the model can predict a continuous sequence of masked positions non-autoregressively, as shown in Fig. {loss of model}. This approach, compared to the two-forward method, avoids mixing with the ground truth with more than one forward passing.

Another disadvantage of using the forward pass twice is that in the first forward pass, the tokens predicted by this type of model are all based on ground truth and do not involve token-by-token prediction based on the previously predicted token~\cite{}. When input into the second forward pass, it's more likely that the replacement words for two adjacent tokens will be discontinuous.
In contrast, the mask-based approach in Non-Autoregressive Transformer (NAT) allows for step-by-step prediction for adjacent masked positions.
